PolyQEnt: A Polynomial Quantified Entailment Solver

Polynomial quantified entailments with existentially and universally quantified variables arise in many problems of verification and program analysis. We present PolyQEnt which is a tool for solving polynomial quantified entailments in which variables on both sides of the implication are real valued or unbounded integers. Our tool provides a unified framework for polynomial quantified entailment problems that arise in several papers in the literature. Our experimental evaluation over a wide range of benchmarks shows the applicability of the tool as well as its benefits as opposed to simply using existing SMT solvers to solve such constraints.

==> problemStatement.tex <==
\section{Problem Statement} \label{sec:problem}

\def\bluecolor{\color{blue}}
\def\blackcolor{\color{black}}


\noindent We start by providing In program analysis, the problem at hand is often reduced to solving a set of \emph{Horn clauses} whose structure depends on the considered class of programs and specifications. Informally speaking, a Horn clause is an implication $\phi \Rightarrow \psi$ where $\phi$ and $\psi$ are logical expressions over program variables. More formally, if the program at hand has a set of variables $V=\{v_1,v_2, \dots, v_n\}$, a horn clause is any formula of the following structure:
\[
[\forall v_1 \in R_1, v_2 \in R_2,\dots, v_n \in R_n; \phi \Rightarrow \psi]
\]
where $R_i$ is the domain of the $i$-th variable in the program. 

\noindent Given a class of programs $\mathcal{P}$ and a specification (either qualitative e.g. termination or quantitative e.g. cost), a \emph{Template Based Certificate Synthesis} method works as follows: 
\begin{enumerate}
    \item Define a certificate $\Psi(P)$ for any $P \in \mathcal{P}$ such that existence of $\Psi(P)$ would imply the desired result regarding the specification on $P$. 
    \item Fix a template $T$ for $\Psi$.
    \item Reduce the problem of finding such $T$ to solving a set of Horn clauses. 
    \item Solve the set of Horn clauses. 
\end{enumerate}

\noindent The above schema can be found in many previous works e.g. \cite{Chatterjee16,Chatterjee20,Zikelic22}. In many cases, the programs are considered to be polynomial (i.e. every arithmetic expression in the program is assumed to be a polynomial in program variables) and the templates fixed in the second step are also polynomials with unknown coefficients. This yields Horn clauses where both the antecedent and the consequent are polynomial expressions and some variables (the ones in the template) are globally existentially quantified. We refer to such clauses as \emph{Polynomial Horn Clauses}. Example \ref{example:schema} illustrates an instance of this schema. 

\begin{figure}[t]
	\centering
	\begin{subfigure}[t]{0.40\textwidth}
		\begin{lstlisting}[frame=none,numbers=none,escapechar=@,mathescape=true]
Invariant: 
  -1024 $\leq$ x $\leq$ 1023
$l_1$:  while x $ \geq$ 1 do
      x := x-1
   done
$l_t$:
		\end{lstlisting}
	\end{subfigure}
	\hfill
        \begin{subfigure}[t]{0.53\textwidth}
        \[
        \hspace{-4cm}
        \begin{split}
        &~~~\exists \blueit{c_1,c_2,c_3,c_4} \in \mathbb{R}\\
            &\begin{cases}
                 \forall x \in \R, \Big(-1024 \leq x \leq 1023 \Rightarrow \blueit{c_1} x + \blueit{c_2} \geq 0 \Big) \\
                  \forall x \in \R, \Big(-1024 \leq x \leq 1023 \wedge x \geq 1 \\ 
                  ~~~~~\Rightarrow \blueit{c_1} (x-1) + \blueit{c_2} \geq 0 \wedge \blueit{c_1} (x-1) + \blueit{c_2} \leq \blueit{c_1} x + \blueit{c_2} - 1 \Big) \\ 
                  \forall x \in \R, \Big(-1024 \leq x \leq 1023 \wedge x < 1 \\~~~~~ \Rightarrow \blueit{c_3} x + \blueit{c_4} \geq 0 \wedge \blueit{c_3} x + \blueit{c_4} \leq \blueit{c_1} x + \blueit{c_2} -1 \Big)
            \end{cases}
        \end{split}
        \]
        \end{subfigure}
        \caption{A simple program (left) and the corresponding Horn clauses for a ranking function that proves termination (right).}
        \label{fig:example}
\end{figure}
    
\begin{example} \label{example:schema}
Consider the program in Fig. \ref{example:schema} (left) and termination as a specification. We describe the four steps of the template-based method:
\begin{enumerate}
    \item Ranking functions are a sound and complete certificate for termination. 
    \item To find such a function, we first put templates at desirable locations in the program. In the example above, for every location $l$ we fix a template ranking function $T_l$ as follows:
\[
    T_l(x) = \begin{cases}
        c_1 x + c_2 & \textit{ if ~} l = l_1 \\
        c_3 x + c_4 & \textit{ if ~} l = l_t
    \end{cases}
\]
 where $c_1,c_2,c_3$ and $c_4$ are the unknown template variables.
    \item The polynomial Horn clauses shown in Fig. \ref{example:schema} (right) imply $T$ being a ranking function. 
    \item One can feed the set of Horn clauses directly into an SMT solver to obtain a valuation of $c$ variables that represent a correct ranking function. \qed
 \end{enumerate} 
\end{example}

\noindent \polyhorn\ is a tool that given a set of polynomial Horn clauses containing some unknown variables (in the form of (\ref{eq:input})), uses Positivestellensatz (for details see Section \ref{sec:positivestellensatz}) to convert it into a fully existentially quantified quadratic formula in real (or if user demands, integer) arithmetic and solves it using state-of-the-art SMT solvers. 

\begin{equation} \label{eq:input}
    \exists c_1, \dots, c_n \in \R; \bigwedge \big(\forall x_1, \dots x_m \in \R; \phi \Rightarrow \psi\big)
\end{equation}

\begin{remark}[Comparison To CHC Solving] \label{remark:chc}
    The problem of solving constrained Horn clauses (CHCs) \cite{Grebenshchikov12,Gurfinke22,Gurfinke19} is fundamentally different from the problem considered here. In CHC solving, the goal is to find functions from program valuations to booleans. For example, if in example \ref{example:schema} the goal was to find a loop invariant, we could fix a function template $inv: \R \to \{true,false\}$ and write CHCs that imply $inv(x)$ being a loop invariant. This does not assume any structure for $inv$. However, in our case, \polyhorn\ looks for a valuation of the existentially quantified \emph{template variables} that might be used in the presentation of a non-boolean function (e.g. in the example above, they are coefficients of a ranking function).
\end{remark}

==> resources/table-AST.tex <==
\begin{table}[t]
	\centering
	\texttt{
        \resizebox{\textwidth}{!}
		{
			\fontsize{6pt}{7pt}\selectfont
                \begin{tabular}{|P{18mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{10mm}|P{10mm}|}
                    \hline 
                     \multirow{2}{*}{Benchmark set} & \multicolumn{3}{c|}{Base} & \multicolumn{3}{c|}{Base+\satheu} & \multicolumn{3}{c|}{Base+\coreheu} & \multicolumn{3}{c|}{Base+\satheu+\coreheu} & \multirow{2}{*}{Dir. Z3} & \multirow{2}{*}{Dir. CVC5}\\
                     \cline{2-13}
                     & MS 5 & Z3 & U. & MS 5 & Z3 & U. & MS 5 & Z3 & U.  & MS 5 & Z3 & U. & &
                     \\
                     \hline 
                     From \cite{Wang19} & 7 & 6 & 7 & 7 & 6 & 7 & 7 & 6 & 7 & 7 & 5 & 7 & 0 & 0 \\
                     \hline 
                     From \cite{Kura19} & 6 & 5 & 6 & 5 & 6 & 6 & 5 & 4 & 5 & 6 & 4 & 6 & 0 & 0\\
                     \hline 
                     \hline 
                     Avg. Time (s) & 10.4 &	6.1 &	10.4 &	9.5 &	3.5 &	9.7 &	10.1 &	3.4 &	10.1 &	10.9 &	2.0 &	10.9 & NA & NA \\
                     \hline 
                \end{tabular}
            }
        }
        \caption{Results on the second benchmark set.}
        \label{table:AST}
        \vspace{-1em}
\end{table}

% 300 seconds:
% \begin{table}
% 	\vspace{-1em}
% 	\centering
% 	\texttt{
%         \resizebox{\textwidth}{!}
% 		{
% 			\fontsize{6pt}{7pt}\selectfont
%                 \begin{tabular}{|P{18mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{10mm}|}
%                     \hline 
%                      \multirow{2}{*}{Benchmark set} & \multicolumn{3}{c|}{Base} & \multicolumn{3}{c|}{Base+\satheu} & \multicolumn{3}{c|}{Base+\coreheu} & \multicolumn{3}{c|}{Base+\satheu+\coreheu} & \multirow{2}{*}{Direct Z3}\\
%                      \cline{2-13}
%                      & MS 5 & Z3 & U. & MS 5 & Z3 & U. & MS 5 & Z3 & U.  & MS 6 & Z3 & U. & 
%                      \\
%                      \hline 
%                      From \cite{Wang19} & 7 & 6 & 7 & 7 & 5 & 7 & 7 & 7 & 7 & 7 & 5 & 7 & 0 \\
%                      \hline 
%                      From \cite{Kura19} & 6 & 5 & 6 & 5 & 6 & 6 & 5 & 5 & 6 & 6 & 5 & 6 & 0\\
%                      \hline 
%                      \hline 
%                      Avg. Time (s) & 22.6 & 8.0 & 16.8 & 20.7 & 6.8 & 16.4 & 19.1 & 20.1 & 15.4 & 22.6 &	10.9 & 17.7 & NA \\
%                      \hline 
%                 \end{tabular}
%             }
%         }
%         \caption{Results obtained by running the experiments on the second benchmark set}
%         \label{table:AST}
% \end{table}

==> resources/table-synth.tex <==
\begin{table}[t]
	\centering
\vspace{-4mm}
	\texttt{
        \resizebox{\textwidth}{!}
		{
			\fontsize{6pt}{7pt}\selectfont
                \begin{tabular}{|P{18mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{10mm}|P{10mm}|}
                    \hline 
                     \multirow{2}{*}{Benchmark Set} & \multicolumn{3}{c|}{Base} & \multicolumn{3}{c|}{Base+\satheu} & \multicolumn{3}{c|}{Base+\coreheu} & \multicolumn{3}{c|}{Base+\satheu+\coreheu} & \multirow{2}{*}{Dir. Z3} & \multirow{2}{*}{Dir. CVC5}\\
                     \cline{2-13}
                     \cline{2-13}
                     & MS 5 & Z3 & U. & MS 5 & Z3 & U. & MS 5 & Z3 & U. & MS 5 & Z3 & U. & &
                     \\
                     \hline 
                     From \cite{Goharshady23} &  28 & 30 & 30 & 28 & 29 & 29 & 28 & 30 & 30 & 28 & 29 & 29 & 24 & 0 \\
                     \hline 
                     \hline 
                     Avg. Time (s) & 3.2 & 2.6 & 2.6 & 2.4 & 2.4 & 2.4 & 2.9 & 2.7 & 2.6 & 2.6 & 2.5 & 2.5 & 14.0 & NA \\
                     \hline 
                \end{tabular}
            }
        }
        \caption{Results on the third benchmark set.}
        \label{table:synth}
        \vspace{-9mm}
\end{table}

% 300s:
% \begin{table}
% 	\vspace{-1em}
% 	\centering
% 	\texttt{
%         \resizebox{\textwidth}{!}
% 		{
% 			\fontsize{6pt}{7pt}\selectfont
%                 \begin{tabular}{|P{18mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{10mm}|}
%                     \hline 
%                      \multirow{2}{*}{Benchmark Set} & \multicolumn{3}{c|}{Base} & \multicolumn{3}{c|}{Base+\satheu} & \multicolumn{3}{c|}{Base+\coreheu} & \multicolumn{3}{c|}{Base+\satheu+\coreheu} & \multirow{2}{*}{Direct Z3}\\
%                      \cline{2-13}
%                      \cline{2-13}
%                      & MS 5 & Z3 & U. & MS 5 & Z3 & U. & MS 5 & Z3 & U. & MS 6 & Z3 & U. & 
%                      \\
%                      \hline 
%                      From \cite{Goharshady23} &  25 & 26 & 26 & 24 & 25 & 25 & 25 & 26 & 26 & 24 & 25 & 25 & 20 \\
%                      \hline 
%                      \hline 
%                      Avg. Time (s) & 6.7 & 6.6 & 6.4 & 6.6 & 6.1 & 6.0 & 6.6 & 6.3 & 6.3 & 6.3 & 6.2 & 6.1 & 8.7\\
%                      \hline 
%                 \end{tabular}
%             }
%         }
%         \caption{Results obtained by running the experiments on the third benchmark set}
%         \label{table:synth}
% \end{table}

==> resources/table-termcomp.tex <==
\begin{table}[t]
	\centering
	\texttt{
        \resizebox{\textwidth}{!}
		{
			\fontsize{6pt}{7pt}\selectfont
                \begin{tabular}{|P{18mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{10mm}|P{10mm}|}
                    \hline 
                     \multirow{2}{*}{Specification} & \multicolumn{3}{c|}{Base} & \multicolumn{3}{c|}{Base+\satheu} & \multicolumn{3}{c|}{Base+\coreheu} & \multicolumn{3}{c|}{Base+\satheu+\coreheu} & \multirow{2}{*}{Dir. Z3} & \multirow{2}{*}{Dir. CVC5}\\
                     \cline{2-13}
                     & MS 5 & Z3 & U. & MS 5 & Z3 & U. & MS 5 & Z3 & U.  & MS 5 & Z3& U. & &
                     \\
                     \hline 
                     Termination & 44 & 154 & 154 & 148 & 153 & 153 & 43 & 109 & 113 & 125 & 132 & 145 & 103 & 9 \\
                     \hline 
                     Non-Termination & 72 & 76 & 78 & 101 & 87 & 103 & 61 & 75 & 76 & 81 & 82 & 89 & 39 & 9 \\
                     \hline 
                     \hline 
                     Avg. Time (s) & 4.4 & 3.9   & 1.6 &	0.5 &	2.5 &	0.5 &	4.3 &	3.5 &	3.4 &	2.7 &	3.7 &	3.6 &	1.6 & 19.4 \\
                     \hline
                \end{tabular}
            }
        }
    \caption{Summary of our results on TermComp benchmarks. The \texttt{Base} column shows the results of \polyqent\ without any heuristics. The next 3~columns enable heuristics \satheu (Assume-SAT) and \coreheu (UNSAT Core). The `Dir. Z3' and `Dir. CVC5' columns summarize the results obtained by applying Z3 and CVC5 directly. For each setting, we show the number of instances solved by MathSAT 5 (\texttt{MS 5}), Z3 and their union (\texttt{U.}).}
    \label{table:termcomp}
    \vspace{-4mm}
\end{table}

% 300s
% \begin{table}[h]
% 	\centering
% 	\texttt{
%         \resizebox{\textwidth}{!}
% 		{
% 			\fontsize{6pt}{7pt}\selectfont
%                 \begin{tabular}{|P{18mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{5mm}|P{10mm}|}
%                     \hline 
%                      \multirow{2}{*}{Specification} & \multicolumn{3}{c|}{Base} & \multicolumn{3}{c|}{Base+\satheu} & \multicolumn{3}{c|}{Base+\coreheu} & \multicolumn{3}{c|}{Base+\satheu+\coreheu} & \multirow{2}{*}{Direct Z3}\\
%                      \cline{2-13}
%                      & MS 5 & Z3 & U. & MS 5 & Z3 & U. & MS 5 & Z3 & U.  & MS 6 & Z3& U. & 
%                      \\
%                      \hline 
%                      Termination & 55 & 151 & 151 & 148 & 149 & 152 & 47 & 124 & 125 & 125 & 131 & 146 & 38 \\
%                      \hline 
%                      Non-Termination & 77 & 88 &	90 & 101 & 92 & 103 & 66 & 83 &	87 & 81 & 86 & 95 & 45 \\
%                      \hline 
%                      \hline 
%                      Avg. Time (s) & 5.2 & 6.5 & 4.7 & 1.0 & 5.7 & 0.8 & 7.7 & 11.7 & 11.4 & 5.5 & 6.0 & 5.8 & 5.3 \\
%                      \hline
%                 \end{tabular}
%             }
%         }
    
%     \caption{Summary of experiments on TermComp benchmarks. The \texttt{Base} column represents the usage of Positivestellensatz as described in \cite{AsadiC0GM21} and each of the next 3 columns is for a specific setting of heuristics. The `Direct Z3' column summarises the results obtained by applying Z3 directly to solve the quantifier elimination instance. For each setting of \polyhorn, we show the number of instances solved by MathSAT 5 (\texttt{MS 5}), Z3 and their union (\texttt{U.}) where for each solved instance, we only consider the faster solver.}
%     \label{table:termcomp}
% \end{table}

==> resources/toolOverview.tex <==
\section{Tool Overview}\label{sec:overview}

\noindent In this section, first, we provide background of the algebraic geometry theorems we used. Then, we present an overview of the design of \polyhorn\ and the heuristics that are implemented.

\subsection{Overview of Positivstellens\"atze} \label{sec:positivestellensatz} % putinar ...,
In this section, we sketch an overview of the theories used by \polyhorn\ in order to convert the input set of polynomial Horn clauses to an instance of quadratic programming.

\smallskip\noindent{\em Theorems description.} There are three main theorems from algebraic geometry that are implemented in \polyhorn. Each of these theorems, considers a Horn clause of the following form:
\begin{equation} \label{eq:linear-example}
    \Big(f_1(V) \geq 0 \wedge f_2(V) \geq 0 \dots f_n(V) \geq 0 \Big) \Rightarrow g(V) \geq 0
\end{equation}
where all $f_1, f_2, \dots f_n$ and $g$ are polynomials in $V$ (possibly with unknown coefficients). It then obtains a set of necessary and sufficient constraints over coefficients of $f_i$s and $g$ for implying $(\ref{eq:linear-example})$. We will go through each and describe their use cases and limitations. For a full description over the theories, we refer the reader to \cite{AsadiC0GM21}.

\begin{itemize}
    \item \textbf{Farkas Lemma \cite{farkas02,matouvsek07}.} In case all $f_i$ and $g$ functions are linear in $V$, Farkas Lemma states that the Horn clause holds if and only if, either (i) $g$ is a non-negative linear combination of $f_i$ functions or (ii) the LHS of the Horn clause is unsatisfiable, or equivalently $-1$ is a linear combination of $f_i$ functions. 
    \item \textbf{Handelman's Positivestellensatz \cite{handelman88}.} In case all $f_i$ functions are linear in $V$ while $g$ is a polynomial, Handelman's positivestellensatz states that the Horn clause holds if and only if either (i) $g$ is the sum of several (possibly 0) products of $f_i$ functions or (ii) the LHS of the Horn clause is unsatisfiable, or equivalently $-1$ can be obtained from $f_i$ function in a similar manner.
    \item \textbf{Putinar's Positivestellensatz \cite{putinar93}.} In case all $f_i$ and $g$ functions are polynomials in $V$, Putinar's positivestellensatz states that either (i) $g$ is a sum of $f_i$ functions each multiplied by a sum-of-squares polynomial, or (ii) the LHS of the Horn clause is unsatisfiable, or equivalently $-1$ can be obtained from $f_i$ function in a similar manner.
\end{itemize}

\noindent Above we briefly described the theories related to non-strict inequalities. However, \cite{AsadiC0GM21} also explains how strict inequalities are handled. 

\noindent The described theorems convert the given Horn clause to a system of quadratic inequalities that are independent from $V$. Given a set of Horn clauses in the form of (\ref{eq:input}), \polyhorn\ applies a pre-specified theorem on each Horn clause and conjuncts the resulting quadratic systems to achieve a fully existentially quantified formula. 

\subsection{Tool Architecture} 

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{resources/polyhorn.drawio.png}
    \caption{Tool Overview}
    \label{fig:overview}
\end{figure}

\smallskip\noindent{\em Architecture.} An overview of \polyhorn\ is depicted in Figure \ref{fig:overview}. 
The tool takes as input a set of polynomial Horn clauses in the form of (\ref{eq:input}) in SMT-LIB format \cite{BarFT-SMTLIB} alongside a
config file in \texttt{.json} format. Examples are provided in the tool's repository. Note that we do not assume any structure on the logical format of the Horn clauses, i.e. the RHS and the LHS of a Horn Clause can have arbitrary \texttt{and} and \texttt{or} statements. The input files are then parsed and, based on the specifications in the config file, \polyhorn\ applies the required theorems to obtain a fully existential polynomial formula and feeds the formula to an SMT-solver. In case the ``UNSAT Core" heuristic is used, the tool will further process the output of the SMT-solver (see section \ref{subsec:heus} for details). Finally, the output of \polyhorn\ is one of (1) \texttt{SAT} with a valuation for the unknown variables, (2) \texttt{UNSAT} if the result of applying the theorem specified in the config file is proved unsatisfiable by the SMT-solver, or (3) \texttt{Unknown} if the SMT-solver returns unknown.
%Finally, after applying theorems and solvers, the tool outputs one of the (1) SAT with the satisfied model, 
%(2) UNSAT, and (3) unknown. The unknown output means that the SMT solver has failed to solve. In the following we will explain each part of the tool with more details.

%The config file must specify a Positivestellensatz (Farkas, Handelman or Putinar), values of its parameters, the heuristics to be applied, the solver to be used (Z3 or MathSAT) and a directory for storing the obtained system of inequalities after applying the theorem.

\smallskip\noindent{\em Configuration File.}
 A config file for a run of \polyhorn\ describes the features that should be used and their required parameters. It should be a \texttt{.json} file specifying (1) a Positivestellensatz (\texttt{farkas}, \texttt{handelman} or \texttt{putinar}), (2) parameters of the Positivestellensatz, (3) which (if any) heuristics to apply, (4) an SMT-solver to be used at the end (\texttt{mathsat} \cite{cimatti2013mathsat5} or \texttt{z3} \cite{de2008z3}), and (5) whether the system of inequalities obtained after applying the Positivestellensatz should be solved using real or integer arithmetic.

\begin{remark}
    We have integrated the commands for running Z3 and MathSAT5 into \polyhorn. However, \polyhorn\ also stores the obtained existential system of inequalities in SMTLIB format which can be fed to any SMT-solver.
\end{remark}


%\paragraph{SMT Solvers} An SMT solver should be fed to our tool for solving Existential quantified formulas where the formula can be disjunctions and conjunctions of polynomial inequalities. The final output of our tool would be the output of this solver. In the case of SAT, the solver would also provide a model which will be the witness for satisfiability of the input.

%\begin{example}
%    ...
%\end{example}


% \begin{itemize}
%     \item describe the pic
%     \item input syntax
%     \item solvers
%     \item describe the config
%     \item one example
% \end{itemize}

\subsection{Heuristics}
\label{subsec:heus}
\noindent Two heuristics are impletemeted in \polyhorn\ which we will briefly discuss in this section. %We implemented two heuristics: Assume SAT and UNSAT core.

\smallskip\noindent{\em Assume-SAT.} This heuristic assumes satisfiability of the premise for each Horn clause $\phi \Rightarrow \psi$. 
%So, instead of considering all the three disjunctions when applying the Positivestellensatz \todoMK{should make clear}, the tool only considers the one where $\phi$ is assumed to be satisfying.
Basically, this heuristic ignores the possibility of $\phi$ being unsatisfiable. Applying this heuristic comes at the cost of losing completeness claims. However, soundness will remain intact, i.e. any model found with this heuristic, is a model for the system obtained without this heuristic. This heuristic reduces the size of the obtained system of inequalities which makes SMT-solvers extremely more efficient.  %Assume-SAT is a classic heuristic that leads to smaller, and so faster system of equations for the SMT solver.

\smallskip\noindent{\em UNSAT Core.}
In \cite{Goharshady23} authors introduce a heuristic which looks like the opposite of abstraction-refinement. The idea is, using Positivestellensatz introduces a lot of new variables which in real-world examples should be set to 0. In order to guide the SMT-solver towards these solutions, for each existential variable $t$, we first add $t=0$ to the system of inequalities and feed it to the SMT-solver. If the SMT-solver returns \texttt{SAT}, then the original system is satisfiable as well, otherwise, both Z3 and MathSAT5 can return an unsatifsiability core, a subset of constraints that are unsatisfiable themselves. If the core contains none of the newly added constraints, it implies that the original system was unsatifiable, otherwise \polyhorn\ removes those $t=0$ constraints that are in the core and repeats. 

%This heuristic benefits from a feature of SMT solvers called "unsat core". With "unsat core", in the case of unsatisfiability, the SMT solver returns an unsatisfiability core containing the equations that lead the system to be unsatisfiable. This heuristic was introduced in\cite{???}. Using this heuristic, our tool sets all the variables to 0 and feeds the system to the SMT solver. Then, in case of unsatisfiability, our tool will remove zeroness of the variables in the "unsat core" and will keep doing this until either we find a satisfiable system or no more zero variable exists. Obviously, this heuristics does not effect soundness and completeness of our tool.

\noindent See section \ref{sec:evaluation} for a detailed analysis on the effects of applying these heuristic.

==> toolOverview.tex <==
\section{Tool Overview}\label{sec:overview}

\noindent In this section, first, we provide background of the algebraic geometry theorems we used. Then, we present an overview of the design of \polyhorn\ and the heuristics that are implemented.

\subsection{Overview of Positivstellens\"atze} \label{sec:positivestellensatz} % putinar ...,
In this section, we sketch an overview of the theories used by \polyhorn\ in order to convert the input set of polynomial Horn clauses to an instance of quadratic programming.

\smallskip\noindent{\em Theorems description.} There are three main theorems from algebraic geometry that are implemented in \polyhorn. Each of these theorems, considers a Horn clause of the following form:
\begin{equation} \label{eq:linear-example}
    \Big(f_1(V) \geq 0 \wedge f_2(V) \geq 0 \dots f_n(V) \geq 0 \Big) \Rightarrow g(V) \geq 0
\end{equation}
where all $f_1, f_2, \dots f_n$ and $g$ are polynomials in $V$ (possibly with unknown coefficients). It then obtains a set of necessary and sufficient constraints over coefficients of $f_i$s and $g$ for implying $(\ref{eq:linear-example})$. We will go through each and describe their use cases and limitations. For a full description over the theories, we refer the reader to \cite{AsadiC0GM21}.

\begin{itemize}
    \item \textbf{Farkas Lemma \cite{farkas02,matouvsek07}.} In case all $f_i$ and $g$ functions are linear in $V$, Farkas Lemma states that the Horn clause holds if and only if, either (i) $g$ is a non-negative linear combination of $f_i$ functions or (ii) the LHS of the Horn clause is unsatisfiable, or equivalently $-1$ is a linear combination of $f_i$ functions. 
    \item \textbf{Handelman's Positivestellensatz \cite{handelman88}.} In case all $f_i$ functions are linear in $V$ while $g$ is a polynomial, Handelman's positivestellensatz states that the Horn clause holds if and only if either (i) $g$ is the sum of several (possibly 0) products of $f_i$ functions or (ii) the LHS of the Horn clause is unsatisfiable, or equivalently $-1$ can be obtained from $f_i$ function in a similar manner.
    \item \textbf{Putinar's Positivestellensatz \cite{putinar93}.} In case all $f_i$ and $g$ functions are polynomials in $V$, Putinar's positivestellensatz states that either (i) $g$ is a sum of $f_i$ functions each multiplied by a sum-of-squares polynomial, or (ii) the LHS of the Horn clause is unsatisfiable, or equivalently $-1$ can be obtained from $f_i$ function in a similar manner.
\end{itemize}

\noindent Above we briefly described the theories related to non-strict inequalities. However, \cite{AsadiC0GM21} also explains how strict inequalities are handled. 

\noindent The described theorems convert the given Horn clause to a system of quadratic inequalities that are independent from $V$. Given a set of Horn clauses in the form of (\ref{eq:input}), \polyhorn\ applies a pre-specified theorem on each Horn clause and conjuncts the resulting quadratic systems to achieve a fully existentially quantified formula. 

\subsection{Tool Architecture} 

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{resources/polyhorn.drawio.png}
    \caption{Tool Overview}
    \label{fig:overview}
\end{figure}

\smallskip\noindent{\em Architecture.} An overview of \polyhorn\ is depicted in Figure \ref{fig:overview}. 
The tool takes as input a set of polynomial Horn clauses in the form of (\ref{eq:input}) in SMT-LIB format \cite{BarFT-SMTLIB} alongside a
config file in \texttt{.json} format. Examples are provided in the tool's repository. Note that we do not assume any structure on the logical format of the Horn clauses, i.e. the RHS and the LHS of a Horn Clause can have arbitrary \texttt{and} and \texttt{or} statements. The input files are then parsed and, based on the specifications in the config file, \polyhorn\ applies the required theorems to obtain a fully existential polynomial formula and feeds the formula to an SMT-solver. In case the ``UNSAT Core" heuristic is used, the tool will further process the output of the SMT-solver (see section \ref{subsec:heus} for details). Finally, the output of \polyhorn\ is one of (1) \texttt{SAT} with a valuation for the unknown variables, (2) \texttt{UNSAT} if the result of applying the theorem specified in the config file is proved unsatisfiable by the SMT-solver, or (3) \texttt{Unknown} if the SMT-solver returns unknown.
%Finally, after applying theorems and solvers, the tool outputs one of the (1) SAT with the satisfied model, 
%(2) UNSAT, and (3) unknown. The unknown output means that the SMT solver has failed to solve. In the following we will explain each part of the tool with more details.

%The config file must specify a Positivestellensatz (Farkas, Handelman or Putinar), values of its parameters, the heuristics to be applied, the solver to be used (Z3 or MathSAT) and a directory for storing the obtained system of inequalities after applying the theorem.

\smallskip\noindent{\em Configuration File.}
 A config file for a run of \polyhorn\ describes the features that should be used and their required parameters. It should be a \texttt{.json} file specifying (1) a Positivestellensatz (\texttt{farkas}, \texttt{handelman} or \texttt{putinar}), (2) parameters of the Positivestellensatz, (3) which (if any) heuristics to apply, (4) an SMT-solver to be used at the end (\texttt{mathsat} \cite{cimatti2013mathsat5} or \texttt{z3} \cite{de2008z3}), and (5) whether the system of inequalities obtained after applying the Positivestellensatz should be solved using real or integer arithmetic.

\begin{remark}
    We have integrated the commands for running Z3 and MathSAT5 into \polyhorn. However, \polyhorn\ also stores the obtained existential system of inequalities in SMTLIB format which can be fed to any SMT-solver.
\end{remark}


%\paragraph{SMT Solvers} An SMT solver should be fed to our tool for solving Existential quantified formulas where the formula can be disjunctions and conjunctions of polynomial inequalities. The final output of our tool would be the output of this solver. In the case of SAT, the solver would also provide a model which will be the witness for satisfiability of the input.

%\begin{example}
%    ...
%\end{example}


% \begin{itemize}
%     \item describe the pic
%     \item input syntax
%     \item solvers
%     \item describe the config
%     \item one example
% \end{itemize}

\subsection{Heuristics}
\label{subsec:heus}
\noindent Two heuristics are impletemeted in \polyhorn\ which we will briefly discuss in this section. %We implemented two heuristics: Assume SAT and UNSAT core.

\smallskip\noindent{\em Assume-SAT.} This heuristic assumes satisfiability of the premise for each Horn clause $\phi \Rightarrow \psi$. 
%So, instead of considering all the three disjunctions when applying the Positivestellensatz \todoMK{should make clear}, the tool only considers the one where $\phi$ is assumed to be satisfying.
Basically, this heuristic ignores the possibility of $\phi$ being unsatisfiable. Applying this heuristic comes at the cost of losing completeness claims. However, soundness will remain intact, i.e. any model found with this heuristic, is a model for the system obtained without this heuristic. This heuristic reduces the size of the obtained system of inequalities which makes SMT-solvers extremely more efficient.  %Assume-SAT is a classic heuristic that leads to smaller, and so faster system of equations for the SMT solver.

\smallskip\noindent{\em UNSAT Core.}
In \cite{Goharshady23} authors introduce a heuristic which looks like the opposite of abstraction-refinement. The idea is, using Positivestellensatz introduces a lot of new variables which in real-world examples should be set to 0. In order to guide the SMT-solver towards these solutions, for each existential variable $t$, we first add $t=0$ to the system of inequalities and feed it to the SMT-solver. If the SMT-solver returns \texttt{SAT}, then the original system is satisfiable as well, otherwise, both Z3 and MathSAT5 can return an unsatifsiability core, a subset of constraints that are unsatisfiable themselves. If the core contains none of the newly added constraints, it implies that the original system was unsatifiable, otherwise \polyhorn\ removes those $t=0$ constraints that are in the core and repeats. 

%This heuristic benefits from a feature of SMT solvers called "unsat core". With "unsat core", in the case of unsatisfiability, the SMT solver returns an unsatisfiability core containing the equations that lead the system to be unsatisfiable. This heuristic was introduced in\cite{???}. Using this heuristic, our tool sets all the variables to 0 and feeds the system to the SMT solver. Then, in case of unsatisfiability, our tool will remove zeroness of the variables in the "unsat core" and will keep doing this until either we find a satisfiable system or no more zero variable exists. Obviously, this heuristics does not effect soundness and completeness of our tool.

\noindent See section \ref{sec:evaluation} for a detailed analysis on the effects of applying these heuristic.
